Automated Off-Policy Estimator Selection via Supervised Learning

The Off-Policy Evaluation (OPE) problem consists of evaluating the performance of counterfactual policies with data collected by another one. To solve the OPE problem, we resort to estimators, which aim to estimate in the most accurate way possible the performance that the counterfactual policies would have had if they were deployed in place of the logging policy. In the literature, several estimators have been developed, all with different characteristics and theoretical guarantees. Therefore, there is no dominant estimator and each estimator may be the best for different OPE problems, depending on the characteristics of the dataset at hand. Although the selection of the estimator is a crucial choice for an accurate OPE, this problem has been widely overlooked in the literature. We propose an automated data-driven OPE estimator selection method based on supervised learning. In particular, the core idea we propose in this paper is to create several synthetic OPE tasks and use a machine learning model trained to predict the best estimator for those synthetic tasks. We empirically show how our method is able to perform a better estimator selection compared to a baseline method on several real-world datasets, with a computational cost significantly lower than the one of the baseline.

==> notheory.tex <==

In this section, we present a novel approach for solving the Estimator Selection problem, called \textit{\bbextAutoOPE} (\bbAutoOPE). 
% The method is centered around a data-driven machine learning model, specifically a Random Forest, which, for a given OPE task, predicts the MSE of various OPE estimators, selecting the one with the lowest predicted MSE.

% The underlying idea is to leverage a \nico{zero-shot meta-learning} meta-learning phase, in which a learning model is trained in a supervised manner to predict the MSE of an estimator, given a set of features describing the logging dataset and both logging and evaluation policies. \bbAutoOPE will also be able to generalize on new OPE tasks in a zero-shot manner. As a supervised learning model, we use a \textit{Random Forest} \citep{random-forest} because of its high-quality predictions on tabular data and its speed, both in training and inference.
\subsection{Theoretical Motivation}

\bbAutoOPE is theoretically justified by many findings that show how the performance of an OPE estimator is highly dependent on the characteristics of the OPE task at hand \cite{voloshin, robustness-off-policy}.
% The concept behind this approach is the dependence of OPE estimators' performance (MSE) on the OPE task characteristics \cite{voloshin}. We propose using a supervised regression model to learn this relationship.
% \nico{Here elaborate making examples of relation between IPS errors and Renyi divergence}
For instance, \cite{metelli-pois, metelli-jmlr, subgaus} theoretically analyze  \textit{Inverse Propensity Scoring} (IPS) \citep{ips1, ips2}, one of the most used OPE estimators and the basis for many others. 
% IPS aims to de-bias the collected rewards by re-weighting them by the inverse of the logging probability: $\hat{V}_{\text{IPS}}(\pie) = \frac{1}{n_b} \sum_{t=1}^{n_b} \pie(a_t|x_t) r_t / \pi_b(a_t|x_t) $.
\citet{metelli-pois} show that the IPS error is strictly related to the (exponentiated) \textit{\renyi} between the logging and evaluation policies\footnote{The \renyi is a divergence between two probability distributions, and it is defined as 
$ d_r(\pie || \pi_b ) = \log \E_x \E_{\ a \sim \pi_b} \left[ ( \pie(a|x) / \pi_b(a|x))^2 \right] $.}
%\mf{$D$ può facilmente confondersi con la notazione del dataset, si può cambiare questa?}
and provide a finite-sample bound on the absolute estimation error of IPS under standard assumptions:
\[ \abs{\Hat{V}_{\text{IPS}}(\pie) - V(\pie) } \leq \mathcal{O}\left( \sqrt{\frac{\exp (d_r(\pie || \pi_b ))}{n_b}} \right), \]
later also proving that this bound is tight \cite{subgaus}. This theoretical finding, along with many others, shows how the performance of an OPE estimator is strictly related to the characteristics of the OPE task, such as the divergence between the evaluation and the logging policy. 
In other words, we assume that: 
\[
MSE(\hat{V}(\pi_e); \task) = f^*(g(\hat{V}, \task)) \ ,
\]
which means that there is a function $f^*$ that express the relationship between the real error of an estimator on a given OPE task $MSE(\hat{V}(\pi_e); \task)$ and the features $g(\hat{V}, \task)$ of the estimator and the task. For this reason, we propose our \textit{zero-shot meta-learning} approach \citep{finn2018learning}, which we frame as a \textit{supervised learning} problem. 

Let us assume that we have a large variety of tasks at our disposal $\mathcal{M} \coloneqq \{\task^{(1)}, \task^{(2)}, \dots\}$, a set of estimators $\mathcal{V}$, and the feature extraction function $g$. Also, let us assume that we have access to the ground-truth MSE. If we have access to these, we could try to find the function that best predicts the MSE for all tasks and estimators, as a standard supervised problem:
\[
\hat{f} = \arg \min_{f} \sum_{\task \in \mathcal{M}} \sum_{\Hat{V} \in \mathcal{V}} \mathcal{L}\left( MSE(\hat{V}(\pi_e); \task) , f(g(\hat{V}, \task)) \right) \ ,
\]

where $\mathcal{L}$ is a suitable loss. Once we found $\hat{f}$, we can apply it in a zero-shot way whenever we need to perform estimator selection with a new task $\task^{(\text{new})} \notin \mathcal{M}$. Indeed, with $\hat{f}$ we can now estimate the MSE for a given task in this way: 
\[\widehat{MSE}_{\bbAutoOPE}\left(\hat{V}, \task^{(\text{new})}\right) \coloneqq \hat{f}(g(\hat{V}, \task^{(\text{new})})).\]
Hence, we just need to select the estimator that minimizes the MSE estimated by \bbAutoOPE: 
\[\hat{V}^* = \arg \min_{\hat{V} \in \mathcal{V}} \widehat{MSE}_{\bbAutoOPE}\left(\hat{V}, \task^{(\text{new})}\right) .\]

\subsection{Practical Implementation}

However, this approach is feasible if we have access to several OPE tasks, a feature extraction function, and the ground-truth MSE. For this reason, our approach extensively rely on \textit{synthetic data}. Specifically:
% \begin{itemize}
%     \item We generate a meta-dataset $\mathcal{M} \coloneqq \{\task^{(1)}, \task^{(2)}, \dots\}$ composed of several different synthetic OPE tasks. In this way, we have access to the ground-truth MSE. Also, since the objective is to obtain a model that is able to generalize in a zero-shot way, we want to train our model with a large number of OPE tasks. This would be unfeasible using real-world OPE data, which is scarce. We indeed generate 250,000 synthetic OPE tasks. Furthermore, to favor generalization of our model, we create OPE tasks with different numerical characteristics. For more details on the synthetic data generation, we refer to Appendix \ref{app:bb-dataset}.
%     \item Regarding the features $g$, while theoretical results have proven a relation, for instance, with the exponentiated \renyi, we want to take into account a wide selection of possible features. Hence, we designed a total of 43 features. 
%     % Such features include several divergence between policies, number of rounds of the task, and many others. 
%     In particular, we categorize the features into three groups:
%     \begin{enumerate*}[label=(\roman*)]
%         \item Policies-independent features, that describe structural properties of the CB scenario and are unrelated from the specific $\pi_b,\ \pi_e$, \eg the number of rounds, the reward mean and variance, the number of actions.
%         \item Policies-dependent features, such as the dissimilarity between the two policies $\pi_b,\ \pi_e$, measured with different geometrical and statistical distances.
%         \item OPE estimator features, that refer to specific properties of the OPE estimator used in that task, \eg if the estimator is self-normalized, uses importance sampling, employs a reward model, and if so, which one. % model is utilized, if the estimator is sub-gaussian, a switch estimator, or shrinked.
%     \end{enumerate*}
%     See Appendix \ref{app:feat-eng} for their full description. 
%     % \nico{forse qui voglio essere leggermente piu specifico e almeno nominare la categorizzazione delle feature (policy-dep, indep., estimator-dep)}
%     \item The set $\mathcal{V}$ of candidate estimators include several model-free, model-based and hybrid estimators, as done in \cite{saito23}. All the estimators used are described in Appendix \ref{app:ope-est}. 
%     \item As a supervised model $f^*$, we use a \textit{Random Forest} \citep{random-forest} because of its high-quality predictions on tabular data and its speed, both in training and inference. For more details on training and optimization, we refer to Appendix \ref{app:bb-model}.
% \end{itemize}


    \paragraph{Dataset} We generate a meta-dataset $\mathcal{M} \coloneqq \{\task^{(1)}, \task^{(2)}, \dots\}$ composed of several different synthetic OPE tasks. In this way, we have access to the ground-truth MSE. Also, since the objective is to obtain a model that is able to generalize in a zero-shot way, we want to train our model with a large number of OPE tasks. This would be unfeasible using real-world OPE data, which is scarce. We indeed generate 250,000 synthetic OPE tasks. Furthermore, to favor generalization of our model, we create OPE tasks with different numerical characteristics. For more details on the synthetic data generation, we refer to Appendix \ref{app:bb-dataset}.
    \paragraph{Features} Regarding the features $g$, while theoretical results have proven a relation, for instance, with the exponentiated \renyi, we want to take into account a wide selection of possible features. Hence, we designed a total of 43 features. 
    % Such features include several divergence between policies, number of rounds of the task, and many others. 
    In particular, we categorize the features into three groups:
    \begin{enumerate*}[label=(\roman*)]
        \item Policies-independent features, that describe structural properties of the CB scenario and are unrelated from the specific $\pi_b,\ \pi_e$, \eg the number of rounds, the reward variance, the number of actions.
        \item Policies-dependent features, such as the dissimilarity between the two policies $\pi_b,\ \pi_e$, measured with different statistical distances and divergences.
        \item OPE estimator features, that refer to specific properties of the OPE estimator used in that task, \eg if the estimator is self-normalized, or uses importance sampling. % model is utilized, if the estimator is sub-gaussian, a switch estimator, or shrinked.
    \end{enumerate*}
    See Appendix \ref{app:feat-eng} for their full description. 
    % \nico{forse qui voglio essere leggermente piu specifico e almeno nominare la categorizzazione delle feature (policy-dep, indep., estimator-dep)}
    \paragraph{Estimators} The set $\mathcal{V}$ of candidate estimators include several model-free, model-based and hybrid estimators, as done in \cite{saito23}. All the estimators used are described in Appendix \ref{app:ope-est}. 
    \paragraph{Model} As a supervised model $\hat{f}$, we use a \textit{Random Forest} regressor \citep{random-forest} because of its high-quality predictions on tabular data and its speed, both in training and inference. For more details on training and optimization, we refer to Appendix \ref{app:bb-model}.


We recap the \bbAutoOPE method in Algorithms \ref{alg:auto-ope-training} (training of the model) and \ref{alg:auto-ope-selection} (zero-shot estimator selection). 

\begin{algorithm}[t]
\small
\caption{\bbAutoOPE training}
\begin{algorithmic}[1]
\REQUIRE Feature generator $g$, estimator set $\mathcal{V}$
\ENSURE MSE estimator $\widehat{MSE}_{\bbAutoOPE}$
\STATE Generate meta-dataset  $\mathcal{M} \coloneqq \{\task^{(1)}, \task^{(2)}, \dots\}$ (Appendix  \ref{app:bb-dataset})
\STATE $\mathcal{L} \gets$ Random Forest regression loss 
\STATE $\hat{f} \gets \arg \min_{f} \sum_{\task \in \mathcal{M}} \sum_{\Hat{V} \in \mathcal{V}} \mathcal{L}\left( MSE(\hat{V}(\pi_e); \task) , f(g(\hat{V}, \task)) \right)$ (Train the random forest)
\STATE For any $\hat{V}, \task$, define $\widehat{MSE}_{\bbAutoOPE}\left(\hat{V}, \task\right) \coloneqq \hat{f}(g(\hat{V}, \task))$
\RETURN $\widehat{MSE}_{\bbAutoOPE}$
\end{algorithmic}
\label{alg:auto-ope-training}
\end{algorithm}


\begin{algorithm}[t]
\small
\caption{\bbAutoOPE estimator selection}
\begin{algorithmic}[1]
\REQUIRE New OPE task $\task^{(\text{new})}$, estimator set $\mathcal{V}$, MSE estimator $\widehat{MSE}_{\bbAutoOPE}$
\ENSURE Selected estimator $\hat{V}^*$
\STATE $\hat{V}^* \gets \arg \min_{\hat{V} \in \mathcal{V}} \widehat{MSE}_{\bbAutoOPE}\left(\hat{V}, \task^{(\text{new})}\right)$
\RETURN $\hat{V}^*$
\end{algorithmic}
\label{alg:auto-ope-selection}
\end{algorithm}

The \bbAutoOPE approach has several advantages. First of all, it is data-driven: \bbAutoOPE tries to learn the shared patterns in several different synthetic OPE tasks with the objective to generalize to new unseen tasks. For this, we use a Random Forest, which is a powerful and fast model for tabular data.
Furthermore, it is theory-inspired: it stems from theoretical findings to create a data-driven model that takes in input features such as divergences which are proven to be related to the estimator's error, but also features that have no theoretical guarantee at the moment. Thanks to this, we can also provide insights that can shed light on future theoretical findings by analyzing the features that had a significant impact on the model's performance. 
Finally, it is zero-shot. This means that a practitioner can avoid training for each new estimator selection task, leading to a much faster computational time. 

A possible downside of our approach is that we trained \bbAutoOPE on large meta-dataset $\mathcal{M}$ that is synthetic and created a priori, which may not lead to generalization to particular real-world OPE tasks.
% \michael{Parlare di retraining se c'è da considerare un nuovo estimator?}
However, in Section \ref{sec:exp}, we show that \bbAutoOPE generalizes well to unseen real-world OPE tasks with an extensive experimental evaluation on a large number of real-world OPE tasks.
